Anomalies of QFTs from M-theory and Holography

We describe a systematic way of computing the 't Hooft anomalies for continuous symmetries of Quantum Field Theories in even dimensions that can be geometrically engineered from M5-branes. Our approach is based on anomaly inflow, and characterizes the anomaly polynomial of the QFT in terms of the geometric definition of the field theory. In particular, when the QFT admits a holographic dual, the topological data of the solution is sufficient to compute the anomalies of the dual field theory, including finite terms in $N$. We study several classes of examples in four and six dimensions, with or without known M5-brane probe configurations.

==> topmatter.tex <==
\def\check{\textbf{CHECK!}}


%\usepackage{array,setspace,mathrsfs,amsfonts,amsmath,yfonts,dsfont,bbm,colonequals,youngtab,mathabx}
%\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}



%\usepackage{graphicx}
%\usepackage{epsfig}
%\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{hyperref}
%\usepackage[height=8.8in,width=6.45in]{geometry}
%\def\baselinestretch{1.05}

\numberwithin{equation}{section}
\newtheorem{conj}{Conjecture}
\newtheorem{thm}{Theorem}

\def\NO#1#2{{\rm NO}(#1,#2)}
\def\CB#1{$\clubsuit$ {\bf #1} $\clubsuit$}
\def\inc#1{\vcenter{\hbox{\includegraphics[scale=.25]{#1}}}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\ceq{\colonequals}
\def\eqc{\equalscolon}
\def\eqq{\equiv}
\def\leqs{\leqslant}
\def\geqs{\geqslant}
\def\vph{\varphi}
\def\vth{\vartheta}
\def\g{\gamma}
\def\G{\Gamma}
\def\th{\theta}
\def\Th{\Theta}
\def\tpdf{\texorpdfstring}

\DeclarePairedDelimiterX\MeijerM[3]{\lparen}{\rparen}%
{\begin{smallmatrix}#1 \\ #2\end{smallmatrix}\delimsize\vert\,#3}

\def\zeromode#1{o\left(#1\right)}

\newcommand\MeijerG[8][]{%
  G^{\,#2,#3}_{#4,#5}\MeijerM[#1]{#6}{#7}{#8}}

\WithSuffix\newcommand\MeijerG*[7]{%
  G^{\,#1,#2}_{#3,#4}\MeijerM*{#5}{#6}{#7}}


%\def\VnoH{\VV_{\cancel{\rm H}}}
\def\VH{\VV_0}
\def\VnoH{\VV_+}
\def\VSch{\mathcal{V}_{\rm Sch}}

\newcommand{\suup}{2}
\newcommand{\sudown}{1}
\def\diag{\mathop{\mathrm{diag}}\nolimits}
\def\tr{\mathop{\mathrm{tr}}\nolimits}
\def\rank{\mathop{\mathrm{rank}}\nolimits}
\def\CP{\mathbb{CP}}
\def\GL{\mathrm{GL}}
\def\SL{\mathrm{SL}}
\def\SU{\mathrm{SU}}
\def\SO{\mathrm{SO}}
\def\USp{\mathrm{USp}}
\def\UU{\mathrm{U}}
\def\PE{\mathrm{PE}}
\def\bC{\mathbb{C}}
\def\bR{\mathbb{R}}
\def\bZ{\mathbb{Z}}
\def\cH{\mathcal{H}}
\def\cDI{\mathcal{DI}}
\def\cN{\mathcal{N}}
\def\cV{\mathbb{V}}
\def\fk{\mathfrak{k}}
\def\fg{\mathfrak{g}}
\def\fh{\mathfrak{h}}
\def\sN{\text{\sffamily N}}
\def\bra#1{\langle#1|}
\def\ket#1{|#1\rangle}
\def\vev#1{\langle#1\rangle}
\def\Hyp{\mathcal{V}}
\def\half{\frac12}
\def\S{{\mathbb S}}


\def\Vir{{\rm Vir}}
\def\AD{{\rm AD}}
\def \Rf{\mf{R}}

\def \beg#1{\begin{#1}} %This is a hack for my compiler -- doesn't have any adverse effects in general
\def \be{\beg{equation}}
\def \bea{\beg{eqnarray}}
\def \eea{\end{eqnarray}}
\def \ee{\end{equation}}

\def \a{\alpha}
\def \b{\beta}
\def \D{\Delta}

\def \PE{\mathrm{P.E.}}
%\def \NO#1{\mathop{:}\nolimits\!#1\!\mathop{:}\nolimits}
\def \goodchi{\protect\raisebox{1pt}{$\chi$}}
\def \qq{\mathbbmtt{Q}\,}
\def \Qt{\wt\QQ}
\def \St{\wt\SS}
\def \Lh{\widehat{L}}
\def \Lb{\overline{L}}
\def \af{\mf{a}}
\def \df{\mf{d}}
\def \ef{\mf{e}}
\def \gf{\mf{g}}
\def \uf{\mf{u}}
\def \glf{\mf{gl}}
\def \slf{\mf{sl}}
\def \suf{\mf{su}}
\def \sof{\mf{so}}
\def \spf{\mf{sp}}
\def \psuf{\mf{psu}}
\def \uspf{\mf{usp}}
\def \ospf{\mf{osp}}
\def \of{\mf{o}}
\def \ef{\mf{e}}
\def \hhf{\mf{h}}
\def \ceq{\colonequals}
\def \bs#1{$\clubsuit${\bf #1}$\clubsuit$}
\def \restr#1#2{{\left.\kern-\nulldelimiterspace#1\vphantom{\big|}\right|_{#2}}}

\def \Poincare{Poincar\'e}

\def \ll{\lambda}

\def \ba{{\bf a}}
\def \bb{{\bf b}}
\def \bc{{\bf c}}
\def \bd{{\bf d}}

\def \bA{{\bf A}}
\def \bB{{\bf B}}
\def \bC{{\bf C}}
\def \bD{{\bf D}}
\def \bOn{{\bf 1}}
\def \bTw{{\bf 2}}
\def \bTh{{\bf 3}}
\def \bFo{{\bf 4}}
\def \bFi{{\bf 5}}
\def \cd{{\tilde c}}

\def \hf{\frac12}
\def \qt{\frac14}

\def \mf{\mathfrak}
\def \lb{\lbrack}
\def \rb{\rbrack}
\def \nn{\nonumber}
\def \ph{\phantom}
\def \wt{\widetilde}
\def \wh{\widehat}
\def \ol{\overline}
\def \eg{{\it e.g.}}
\def \ie{{\it i.e.}}
\def \cf{{\it cf.}}
\def \Tr{{\rm Tr}}
\def \STr{{\rm STr}}
\def \til{\tilde}
\def \pr{\prime}
\def \zb{{\bar z}}
\def \db{\ol{\partial}}
\def \d{\partial}
\def \dag{\dagger}

\def \Ab{\mathbb{A}}
\def \Cb{\mathbb{C}}
\def \Eb{\mathbb{E}}
\def \Fb{\mathbb{F}}
\def \Hb{\mathbb{H}}
\def \Kb{\mathbb{K}}
\def \Mb{\mathbb{M}}
\def \Nb{\mathbb{N}}
\def \Ob{\mathbb{O}}
\def \Qb{\mathbb{Q}}
\def \Rb{\mathbb{R}}
\def \Sb{\mathbb{S}}
\def \Zb{\mathbb{Z}}


\def \AA{\mathcal{A}}
\def \BB{\mathcal{B}}
\def \CC{\mathcal{C}}
\def \DD{\mathcal{D}}
\def \EE{\mathcal{E}}
\def \FF{\mathcal{F}}
\def \GG{\mathcal{G}}
\def \HH{\mathcal{H}}
\def \II{\mathcal{I}}
\def \JJ{\mathcal{J}}
\def \KK{\mathcal{K}}
\def \LL{\mathcal{L}}
\def \MM{\mathcal{M}}
\def \NN{\mathcal{N}}
\def \OO{\mathcal{O}}
\def \PP{\mathcal{P}}
\def \QQ{\mathcal{Q}}
\def \RR{\mathcal{R}}
\def \SS{\mathcal{S}}
\def \TT{\mathcal{T}}
\def \UU{\mathcal{U}}
\def \VV{\mathcal{V}}
\def \WW{\mathcal{W}}
\def \XX{\mathcal{X}}
\def \YY{\mathcal{Y}}
\def \ZZ{\mathcal{Z}}


\def \RRR{\mathfrak{R}}

